Boosting Path-Sensitive Value Flow Analysis via Removal of Redundant Summaries

Value flow analysis that tracks the flow of values via data dependence is a widely used technique for detecting a broad spectrum of software bugs. However, the scalability issue often deteriorates when high precision (i.e., path-sensitivity) is required, as the instantiation of function summaries becomes excessively time- and memory-intensive. The primary culprit, as we observe, is the existence of redundant computations resulting from blindly computing summaries for a function, irrespective of whether they are related to bugs being checked. To address this problem, we present the first approach that can effectively identify and eliminate redundant summaries, thereby reducing the size of collected summaries from callee functions without compromising soundness or efficiency. Our evaluation on large programs demonstrates that our identification algorithm can significantly reduce the time and memory overhead of the state-of-the-art value flow analysis by 45\% and 27\%, respectively. Furthermore, the identification algorithm demonstrates remarkable efficiency by identifying nearly 80\% of redundant summaries while incurring a minimal additional overhead. In the largest \textit{mysqld} project, the identification algorithm reduces the time by 8107 seconds (2.25 hours) with a mere 17.31 seconds of additional overhead, leading to a ratio of time savings to paid overhead (i.e., performance gain) of 468.48 $\times$. In total, our method attains an average performance gain of 632.1 $\times$.

==> proof.tex <==
\appendix

\begin{theorem}[Soundness]
\label{thm:sound}

Given $V^{N}$ identified, for any function $f \in P$, if a summary $s=(\pi, \phi)$ is being collected and neither $\pi[0]$ nor $\pi[-1]$ appear in $V^{I}$, it must be a non-contributing summary for function $f$. Canceling the corresponding operations does not affect $S(V_{\text{src}}, V_{\text{sink}})$.
\begin{proof}

In Algorithm 1, when collecting the summary $s$ between $V_{h}^{f}$ and $V_{t}^{f}$, if $\pi[0] \notin V_h^{p*} \cup V_t^{p*}$ or $\pi[-1] \notin V_h^{p*} \cup V_t^{p*}$, it indicates that $s$ cannot be reached by any source-sink pairs. Therefore, it does not contribute to any source-sink path. If $\pi[0] \notin V_h^{c*} \cup V_t^{c*}$ or $\pi[-1] \notin V_h^{c*} \cup V_t^{c*} \cup V_{\text{g}}^{*}$, it means that $s$ cannot be used to constrain any source-sink path. Hence, it does not contribute to any condition. In such cases, the collecting operation should be canceled.

In Algorithm 1, when collecting the summary $s$ by concatenating it with the summaries $S^{c}$ cloned from callee functions, following the same judgment conditions as described in the previous case, if it is determined to be a non-contributing summary, the operation of cloning $s^{c}$ should be canceled.
\end{proof}
\end{theorem}

\begin{table}[] \small
\caption{Classification of unsafe sinks (US) and safe sinks (S) reported by Fusion (F), Light-Fusion (LF), and Phasar (P).
}
\label{table:report}
\resizebox{\columnwidth}{!} {
\begin{tabular}{r|rrrl|llll}
\hline
ID & \multicolumn{1}{c}{\#Sinks} & \multicolumn{1}{c}{F-US} & LF-US & \multicolumn{1}{c|}{P-US} & \multicolumn{1}{c}{F-US$\wedge$P-US} & \multicolumn{1}{c}{F-S$\wedge$P-S} & \multicolumn{1}{c}{F-S$\wedge$P-US} & \multicolumn{1}{r}{F-US$\wedge$P-S} \\ \hline
1  & 3184                        & 2                        & 2     & 11                        & 2                                    & 3173                               & 9                                   & 0                                   \\
2  & 3581                        & 9                        & 9     & 86                        & 9                                    & 3,495                              & 77                                  & 0                                   \\
3  & 7657                        & 0                        & 0     & 5                         & 0                                    & 7652                               & 5                                   & 0                                   \\
4  & 4273                        & 1                        & 1     & 261                       & 1                                    & 4012                               & 261                                 & 1                                   \\
5  & 27489                       & 28                       & 28    & 207                       & 28                                   & 27282                              & 186                                 & 7                                   \\
6  & 14490                       & 31                       & 31    & 93                        & 31                                   & 14397                              & 69                                  & 7                                   \\
7  & 49769                       & 26                       & 26    & 378                       & 26                                   & 49391                              & 354                                 & 2                                   \\
8  & 12156                       & 12                       & 12    & 111                       & 12                                   & 12045                              & 101                                 & 2                                   \\
9  & 40888                       & 19                       & 19    & 669                       & 19                                   & 40219                              & 653                                 & 3                                   \\
10 & 3418                        & 8                        & 8     & 217                       & 8                                    & 3201                               & 213                                 & 4                                   \\
11 & 215747                      & 35                       & 35    & 103                       & 35                                   & 215644                             & 68                                  & 0                                   \\
12 & 77705                       & 28                       & 28    & 281                       & 28                                   & 77424                              & 257                                 & 4                                   \\
13 & 146208                      & 79                       & 79    & 3592                      & 79                                   & 142616                             & 3516                                & 3                                   \\
14 & 182621                      & 65                       & 65    & 3902                      & 65                                   & 178719                             & 3839                                & 2                                   \\ \hline
15 & 76727                       & 103                      & 103   & 2382                      & 103                                  & 74345                              & 2289                                & 10                                  \\
16 & 146284                      & 92                       & 92    & 1102                      & 92                                   & 145182                             & 1018                                & 8                                   \\
17 & 215431                      & 168                      & 168   & 2007                      & 168                                  & 213424                             & 1845                                & 6                                   \\ \hline
\end{tabular}
}
\vspace{-0.4cm}
\end{table}
